NPBG++: Accelerating Neural Point-Based Graphics

We present a new system (NPBG++) for the novel view synthesis (NVS) task that achieves high rendering realism with low scene fitting time. Our method efficiently leverages the multiview observations and the point cloud of a static scene to predict a neural descriptor for each point, improving upon the pipeline of Neural Point-Based Graphics in several important ways. By predicting the descriptors with a single pass through the source images, we lift the requirement of per-scene optimization while also making the neural descriptors view-dependent and more suitable for scenes with strong non-Lambertian effects. In our comparisons, the proposed system outperforms previous NVS approaches in terms of fitting and rendering runtimes while producing images of similar quality.

==> src/figures/fig_aggregation.tex <==
\begin{figure*}[ht]
\centering
\includegraphics[width=1.0\textwidth]{img/aggregation.png}
\figcaption{Title.}{Text}
\label{fig:aggregation}
\end{figure*}


==> src/figures/fig_alignment.tex <==
\begin{figure}[ht]
\centering
\includegraphics[width=0.99\columnwidth]{img/alignment.pdf}
\figcaption{The impact of alignment.}{Input view alignment (`I alignment') and rendering alignment (`R alignment') improve the final result for neural-point-based graphics pipelines. The original NPBG\cite{aliev2020neural} corresponds to NPBG with `no R alignment'.}
\label{fig:alignment}
\end{figure}


==> src/figures/fig_comparisons_part2.tex <==
\begin{figure*}[ht]
\centering
\includegraphics[width=0.99\textwidth]{img/comparisons_part2.pdf}
\figcaption{Additional qualitative evaluations.}{Comparisons with otimization-based approaches (NPBG\cite{aliev2020neural}, NeRF\cite{mildenhall2020nerf}) and learning based approaches (IBRNet\cite{wang2021ibrnet}, SVS\cite{riegler2021stable}) on ScanNet\cite{dai2017scannet}, NeRF-Synthetic\cite{mildenhall2020nerf}, DTU\cite{jensen2014large}, H3DS\cite{ramon2021h3d} scenes.}
\label{fig:comparisons_part2}
\end{figure*}


==> src/figures/fig_latency.tex <==
% \begin{figure}[ht]
% \centering
% \includegraphics[width=0.99\columnwidth]{img/latency.pdf}
% \figcaption{Rendering runtime evaluation.}{\todo{Add 800x800 line?} The rendering runtime of our system depends on the number of points in the pointcloud and the image size. E.g. to produce 1920x1080 image using 1 mln points it takes 79.3 ms = 0.05 ms (descriptors calculation step) + 11.51 ms (rasterization step) + 61.23 ms (refinement step) + 6.51 ms (output image alignment). On average descriptors calculation step takes 1\%, rasterization step - 73\%, refinement step - 18\%, output image alignment - 8\% of total time. Measured using nVidia geforce 1080 Ti. \todo{add processing runtime evaluation?} \todo{combine all runtime figures}}
% \label{fig:latency}
% \end{figure}

\begin{figure*}[h]
\centering
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.99\columnwidth]{img/runtime_preparation.pdf}
  \label{fig:sub1}
\end{subfigure}%
\begin{subfigure}{.5\textwidth}
  \centering
  \includegraphics[width=0.99\columnwidth]{img/runtime_test.pdf}
  \label{fig:sub2}
\end{subfigure}
\figcaption{Runtime evaluation.}{\textbf{a)} Single input image processing time (denoted $U$) depends on image size and number of points and includes time for feature extraction plus the time to update intermediate states. If we let $P$ be the time required to obtain the point cloud (e.g. using MVS), and denote with $S$ the time required to compute \Eq{beta_0}, \Eq{beta}, then the $\text{3d modeling stage total runtime is equal to } P + \text{\#images} \times U + S$. $S$ takes from 512 ms to 3059 ms when varying the number of points from 1 mln to 6 mln and does not depend on image size. \textbf{b)}. Rendering time depends on image size and number of points. On average, descriptors calculation step takes 0.05\%, rasterization step - 37.86\%, refinement step - 57.85\%, and output image alignment - 4.24\% of total rendering time during novel view synthesis. In principle, one can accelerate the rasterization step using an OpenGL implementation instead of a PyTorch-based one. The time was measured using Nvidia GeForce 1080 Ti. The refinement step can also potentially be accelerated by using neural architecture search and other common techniques.}
\label{fig:latency}
\end{figure*}

% E.g. to produce 1920x1080 image using 1 mln points it takes 79.3 ms = 0.05 ms (descriptors calculation step) + 11.51 ms (rasterization step) + 61.23 ms (refinement step) + 6.51 ms (output image alignment).

==> src/figures/fig_style_transfer.tex <==
\begin{figure*}[h]
\centering
\includegraphics[width=0.99\textwidth]{img/style_transfer.pdf}
\figcaption{Qualitative results of 3D scene stylization.}{The leftmost column shows one of the input views with the input style image on the top-left corner. The other columns represent the stylization result at different novel views.}
\label{fig:style_transfer}
\end{figure*}


==> src/figures/fig_view_selection.tex <==
\begin{figure}[t]
\centering
\includegraphics[width=0.8\columnwidth]{img/view_selection.pdf}
\figcaption{View selection and cropping.}{During training, we randomly crop a target (reference) patch. a) We select three relevant input views and apply input image alignment. b) We make the crops of size twice larger compared to the target patch. Crops are done so that as many points visible in the target patch (marked with \emph{green} color in the Figure) are projected inside the cropped region. We do not resize crops.}
\label{fig:view_selection}
\end{figure}

% Use "self-contained" caption. It's annoying to dig into the texts and match them to the figures. Ain't nobody got time for that!
% Also, add a figure "caption title" (in bold fonts). It allows readers to navigate through figures quickly.

==> src/tables/tab_comparisons.tex <==
\begin{table*}[ht]
\centering
\input{src/tables/tab_comparisons_nerf_synthetic}
% \bigskip
\input{src/tables/tab_comparisons_scannet}
% \bigskip
\input{src/tables/tab_comparisons_dtu}
% \bigskip
\input{src/tables/tab_comparisons_h3ds}
\figcaption{Detailed quantitative evaluations.}{For each scene, we compute the metrics \cite{zhang2018perceptual} on holdout frames. Subscript \emph{ft} indicates finetuned versions of the methods. In the case of NPBG++$_{\emph{ft}}$ we directly finetune coefficients ($\beta$, $\beta_0$) and the refiner. In the case of NPBG++$_{\emph{ft-system}}$ we finetune the feature extractor, aggregator (MLP: neural basis functions), and refiner.}
\label{tab:comparisons}
\end{table*}

==> src/tables/tab_comparisons_dtu.tex <==
% \begin{table*}[ht]
% \centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccc}
% \toprule
& & & & & & & & & & \\
\toprule
& & \multicolumn{3}{c}{DTU - 110} & \multicolumn{3}{c}{DTU - 114} & \multicolumn{3}{c}{DTU - 118} \\ \cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}
Method & \begin{tabular}[c]{@{}l@{}}Per scene\\ optimization\end{tabular} & \textbf{PSNR}$\uparrow$      & \textbf{SSIM}$\uparrow$      & \textbf{LPIPS}$\downarrow$      & \textbf{PSNR}$\uparrow$      & \textbf{SSIM}$\uparrow$      & \textbf{LPIPS}$\downarrow$      & \textbf{PSNR}$\uparrow$      & \textbf{SSIM}$\uparrow$      & \textbf{LPIPS}$\downarrow$      \\ \midrule
SVS\cite{riegler2021stable} & \xmark        &
19.22       & 0.872     & 0.178     & 
22.04       & 0.893     & 0.165     & 
21.69       & 0.927     & 0.143     \\
IBRNet\cite{wang2021ibrnet} & \xmark        & 
23.77       & 0.923     & 0.238     &
27.42       & 0.910     & 0.231     &
26.24       & 0.938     & 0.225     \\
\textbf{NPBG++ (Ours)} & \xmark &
21.13       & 0.907     & 0.161     & 
24.57       & 0.904     & 0.164     & 
24.00       & 0.933     & 0.137     \\
\cmidrule{1-11}
NPBG\cite{aliev2020neural} & \cmark     & 
24.65           & 0.916         & 0.123         & 
26.74           & 0.891         & 0.137         & 
26.62           & 0.932         & 0.114         \\ 
NeRF\cite{mildenhall2020nerf}   & \cmark    & 
25.55      & 0.917     & 0.194     &
27.42      & 0.894     & 0.217     &
27.78      & 0.928     & 0.182     \\
SVS$_{\emph{ft}}$\cite{riegler2021stable}   & \cmark    & 
17.57       & 0.842     & 0.208     & 
21.57       & 0.860     & 0.192     & 
23.01       & 0.889     & 0.171     \\
IBRNet$_{\emph{ft}}$\cite{wang2021ibrnet}   & \cmark    & 
23.69       & 0.915     & 0.238     &
25.43       & 0.913     & 0.193     &
22.28       & 0.923     & 0.237     \\
\textbf{NPBG++$_{\emph{ft-system}}$ (Ours)}   & \cmark    & 
22.30       & 0.916     & 0.150         & 
25.16       & 0.906     & 0.162         & 
24.70       & 0.935     & 0.128         \\
\textbf{NPBG++$_{\emph{ft}}$ (Ours)}  & \cmark    & 
24.84       & 0.929     & 0.122     & 
26.72       & 0.911     & 0.134     & 
26.67       & 0.945     & 0.113     \\
\bottomrule
\end{tabular}
}
% \figcaption{Quantitative evaluations on DTU scenes.}{For each scene, we compute the metrics \cite{zhang2018perceptual} on holdout frames.}
% \label{tab:comparisons_dtu}
% \end{table*}

==> src/tables/tab_comparisons_h3ds.tex <==
% \begin{table*}[ht]
% \centering
\resizebox{0.8\textwidth}{!}{
\begin{tabular}{lccccccc}
% \toprule
& & & & & & & \\
\toprule
& & \multicolumn{3}{c}{H3DS - 5ae021f2805c0854} & \multicolumn{3}{c}{H3DS - 7dd427509fe84baa} \\ \cmidrule(lr){3-5}\cmidrule(lr){6-8}
Method & \begin{tabular}[c]{@{}l@{}}Per scene\\ optimization\end{tabular} & \textbf{PSNR}$\uparrow$      & \textbf{SSIM}$\uparrow$      & \textbf{LPIPS}$\downarrow$      & \textbf{PSNR}$\uparrow$      & \textbf{SSIM}$\uparrow$      & \textbf{LPIPS}$\downarrow$      \\ \midrule
SVS\cite{riegler2021stable} & \xmark        & 
19.24       & 0.763     & 0.230     &
18.68       & 0.833     & 0.189     \\
IBRNet\cite{wang2021ibrnet} & \xmark        & 
21.23       & 0.756     & 0.303     & 
19.37       & 0.826     & 0.255     \\
\textbf{NPBG++ (Ours)} & \xmark & 
22.26       & 0.782     & 0.202     & 
21.33       & 0.854     & 0.151     \\
\cmidrule{1-8}
NPBG\cite{aliev2020neural} & \cmark     & 
24.59           & 0.783     & 0.170  & 
24.77           & 0.871     & 0.122         \\
NeRF\cite{mildenhall2020nerf}   & \cmark    & 
23.81       & 0.797       & 0.202     &
23.95       & 0.868       & 0.153     \\
SVS$_{\emph{ft}}$\cite{riegler2021stable}   & \cmark    & 
20.95       & 0.738     & 0.206     & 
19.29       & 0.801     & 0.188     \\
IBRNet$_{\emph{ft}}$\cite{wang2021ibrnet}   & \cmark    & 
25.13       & 0.811     & 0.224     & 
24.22       & 0.889     & 0.165     \\
\textbf{NPBG++$_{\emph{ft-system}}$ (Ours)}   & \cmark    & 
24.08       & 0.795     & 0.182         & 
23.49       & 0.876     & 0.127         \\
\textbf{NPBG++$_{\emph{ft}}$ (Ours)}   & \cmark    & 
25.08       & 0.805     & 0.158     & 
24.73       & 0.885     & 0.116     \\
\bottomrule
\end{tabular}
}
% \figcaption{Quantitative evaluations on H3DS scenes.}{For each scene, we compute the metrics \cite{zhang2018perceptual} on holdout frames.}
% \label{tab:comparisons_h3ds}
% \end{table*}

==> src/tables/tab_comparisons_nerf_synthetic.tex <==
% \begin{table*}[ht]
% \centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccc}
\toprule
& & \multicolumn{3}{c}{Nerf-Synthetic - Hotdog} & \multicolumn{3}{c}{Nerf-Synthetic - Ficus} & \multicolumn{3}{c}{Nerf-Synthetic - Mic} \\ \cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}
Method & \begin{tabular}[c]{@{}l@{}}Per scene\\ optimization\end{tabular} & \textbf{PSNR}$\uparrow$      & \textbf{SSIM}$\uparrow$      & \textbf{LPIPS}$\downarrow$      & \textbf{PSNR}$\uparrow$      & \textbf{SSIM}$\uparrow$      & \textbf{LPIPS}$\downarrow$      & \textbf{PSNR}$\uparrow$      & \textbf{SSIM}$\uparrow$      & \textbf{LPIPS}$\downarrow$      \\ \midrule
% NeRF          & 1         & 2         & 3          & 4         & 5         & 6          & 7         & 8         & 9          \\
SVS\cite{riegler2021stable} & \xmark        &
25.70       & 0.933     & 0.107     & 
20.29       & 0.883     & 0.132     & 
22.44       & 0.940     & 0.072     \\
IBRNet\cite{wang2021ibrnet} & \xmark        &
33.33       & 0.969     & 0.144     &
25.47       & 0.926     & 0.186     &
29.60       & 0.969     & 0.140     \\
\textbf{NPBG++ (Ours)} & \xmark &
28.84       & 0.949     & 0.078     & 
22.48       & 0.903     & 0.090     & 
26.87       & 0.957     & 0.045     \\
\cmidrule{1-11}
NPBG\cite{aliev2020neural} & \cmark     & 
32.26       & 0.957     & 0.059         & 
24.71       & 0.920     & 0.078         & 
28.88       & 0.962     & 0.036         \\ 
NeRF\cite{mildenhall2020nerf}   & \cmark    & 
36.08           & 0.975     & 0.045     &
29.29           & 0.958     & 0.049     &
32.10           & 0.977     & 0.030     \\
SVS$_{\emph{ft}}$\cite{riegler2021stable}   & \cmark    & 
26.56       & 0.934     & 0.105     & 
20.62       & 0.879     & 0.128     & 
22.93       & 0.943     & 0.071     \\
IBRNet$_{\emph{ft}}$\cite{wang2021ibrnet}   & \cmark    & 
36.46           & 0.980     & 0.137     &
28.66           & 0.957     & 0.146     &
32.40           & 0.980     & 0.148     \\
\textbf{NPBG++$_{\emph{ft-system}}$ (Ours)}   & \cmark    & 
27.16           & 0.948         & 0.072 &
23.48           & 0.911         & 0.082 & 
28.08           & 0.962         & 0.037 \\
\textbf{NPBG++$_{\emph{ft}}$ (Ours)}   & \cmark    & 
32.31       & 0.964     & 0.050     & 
24.61       & 0.925     & 0.070     & 
29.08       & 0.967     & 0.029     \\
\bottomrule
\end{tabular}
}
% \figcaption{Quantitative evaluations on Nerf-Synthetic scenes.}{For each scene, we compute the metrics \cite{zhang2018perceptual} on holdout frames.}
% \label{tab:comparisons_nerf_synthetic}
% \end{table*}

==> src/tables/tab_comparisons_scannet.tex <==
% \begin{table*}[ht]
% \centering
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccccc}
% \toprule
& & & & & & & & & & \\
\toprule
& & \multicolumn{3}{c}{ScanNet - 0000} & \multicolumn{3}{c}{ScanNet - 0043} & \multicolumn{3}{c}{ScanNet - 0045} \\ \cmidrule(lr){3-5}\cmidrule(lr){6-8}\cmidrule(lr){9-11}
Method & \begin{tabular}[c]{@{}l@{}}Per scene\\ optimization\end{tabular} & \textbf{PSNR}$\uparrow$      & \textbf{SSIM}$\uparrow$      & \textbf{LPIPS}$\downarrow$      & \textbf{PSNR}$\uparrow$      & \textbf{SSIM}$\uparrow$      & \textbf{LPIPS}$\downarrow$      & \textbf{PSNR}$\uparrow$      & \textbf{SSIM}$\uparrow$      & \textbf{LPIPS}$\downarrow$      \\ \midrule
SVS\cite{riegler2021stable} & \xmark  &
22.17       & 0.752 & 0.442 &
21.74       & 0.833 & 0.429 & 
26.06       & 0.727 & 0.465 \\
IBRNet\cite{wang2021ibrnet} & \xmark    & 
19.54       & 0.703 & 0.535 & 
24.42       & 0.859 & 0.434 & 
26.07       & 0.719 & 0.513 \\
\textbf{NPBG++ (Ours)} & \xmark &
20.66        & 0.738        & 0.530 &
22.63        & 0.845        & 0.464 &
26.04        & 0.716        & 0.511         \\
\cmidrule{1-11}
NPBG\cite{aliev2020neural} & \cmark &
22.24    & 0.695     & 0.474 &
25.27    & 0.830     & 0.421 &
27.75    & 0.686     & 0.482         \\
NeRF\cite{mildenhall2020nerf}   & \cmark    & 
22.08      & 0.729    & 0.588         &
25.98      & 0.869    & 0.466         &
29.15      & 0.743    & 0.558        \\
SVS$_{\emph{ft}}$\cite{riegler2021stable}   & \cmark    & 
21.30       & 0.559 & 0.535 &
21.24       & 0.737 & 0.531 &
24.38       & 0.533 & 0.562 \\
IBRNet$_{\emph{ft}}$\cite{wang2021ibrnet} & \cmark    & 
20.14       & 0.714 & 0.528 &
25.56       & 0.868 & 0.427 &
27.57       & 0.741 & 0.523 \\
\textbf{NPBG++$_{\emph{ft-system}}$ (Ours)}   & \cmark    & 
21.04           & 0.738     & 0.517     &
22.31           & 0.846     & 0.454     &
27.08           & 0.720     & 0.498     \\
\textbf{NPBG++$_{\emph{ft}}$ (Ours)}   & \cmark    & 
22.05       & 0.742 & 0.457 &
25.51       & 0.859 & 0.410 &
28.26       & 0.716 & 0.477 \\
\bottomrule
\end{tabular}
}
% \figcaption{Quantitative evaluations on ScanNet scenes.}{For each scene we compute the metrics \cite{zhang2018perceptual} on holdout frames.}
% \label{tab:comparisons_scannet}
% \end{table*}

==> src/tables/tab_num_views.tex <==
\begin{table}[ht]
\centering
\resizebox{0.8\columnwidth}{!}{
\begin{tabular}{cccc}
\toprule
number of views & \textbf{PSNR}$\uparrow$ & \textbf{SSIM}$\uparrow$ & \textbf{LPIPS}$\downarrow$ \\
\midrule
3 & 19.29 & 0.770 & 0.219 \\
5 & 20.34 & 0.790 & 0.198 \\
10 & 20.88 & 0.799 & 0.192 \\
15 & 21.49 & 0.812 & 0.181 \\
22 & 21.80 & 0.818 & 0.177 \\
\bottomrule
\end{tabular}
}
\figcaption{Number of views impact.}{We report metrics averaged across two holdout H3DS scenes. PatchmatchNet \cite{wang2020patchmatchnet} results in bad reconstruction when using a small number of views (5-10). We use the point cloud obtained using all 22 source views.}
\label{tab:num_views}
\end{table}
